text2sdg: An R package to Monitor Sustainable Development Goals from Text

Monitoring progress on the United Nations Sustainable Development Goals (SDGs) is important for both academic and non-academic organizations. Existing approaches to monitoring SDGs have focused on specific data types; namely, publications listed in proprietary research databases. We present the text2sdg package for the R language, a user-friendly, open-source package that detects SDGs in any kind of text data using different existing or custom-made query systems. The text2sdg package thereby facilitates the monitoring of SDGs for a wide array of text sources and provides a much-needed basis for validating and improving extant methods to detect SDGs from text.

==> graveyard.tex <==

 
 The most basic of these systems consist of simple keyword queries that map keywords to SDGs. For example, the query system OSDG \cite[]{Bautista2019} maps the keyword "poverty" to SDG-01. These keywords can also consist of multiple words, e.g., the "extreme poverty" keyword also maps onto SDG-01 in the OSDG system. In contrast to these simple keyword based query systems, there exist more complicated systems that also make use of keywords, but combine these keywords with boolean (and proximity) operators. For example, the SIRIS query system maps the keyword "basic needs" to SDG-01 only if the text also contains one of the following keywords: "poverty", "disadvantaged" or "developping countries.
